AutoGain: Gain Function Adaptation with Submovement Efficiency Optimization

A well-designed control-to-display gain function can improve pointing performance with indirect pointing devices like trackpads. However, the design of gain functions is challenging and mostly based on trial and error. AutoGain is a novel method to individualize a gain function for indirect pointing devices in contexts where cursor trajectories can be tracked. It gradually improves pointing efficiency by using a novel submovement-level tracking+optimization technique that minimizes aiming error (undershooting/overshooting) for each submovement. We first show that AutoGain can produce, from scratch, gain functions with performance comparable to commercial designs, in less than a half-hour of active use. Second, we demonstrate AutoGain's applicability to emerging input devices (here, a Leap Motion controller) with no reference gain functions. Third, a one-month longitudinal study of normal computer use with AutoGain showed performance improvements from participants' default functions.

==> graveyard.tex <==
\section{Practical Deployment}

While useful in applications with dedicated pointers that can be controlled independently from the system cursor, our main objective is to allow constant, personalized gain optimization at operating system level.
Deploying \methodname\ at system level requires 4 elements:
% 
\begin{itemize}
	% 
	\item \emph{Cursor trajectory logging}, which is often trivial.
    % 
    % \item \emph{Input motion logging}, which is sometimes available programmatically or with dedicated hardware \cite{clutching,casiez2011no}. 
    % It can also be approximated from cursor trajectory, provided sufficient knowledge about the current gain function.
    % The same considerations apply to clutching detection: some devices provide contact-up and contact-down events.
    % Otherwise, heuristics like duration thresholds with no input events may provide a satisfactory approximation.
    % 
    % \item \emph{Distinguishing pointing movements} in real time (as opposed to e.g., idle movements or steering), for which various speed-based methods have been proposed \cite{evans12,fittswild}.
    % % Evans \etal{}~\cite{evans12} proposed a real-time method for this end.
    % % 
        \item \emph{Altering the gain function of the system cursor}.
    To disable the system transfer function, we can suppress the low level mouse move messages by using the GlobalMouseKeyHook library (set \texttt{e.Handled} flag set to \texttt{TRUE} within \texttt{WH\_MOUSE\_LL} message handler).
In parallel, we can capture device-level raw input messages using the Microsoft Raw Input API.
% \footnote{\small\url{https://msdn.microsoft.com/en-us/library/windows/desktop/ms645536(v=vs.85).aspx}\normalsize}. 
Then a custom transfer function can be applied on those raw messages, and generates new mouse-move messages by calling the \texttt{SetCursorPos()} function in the Microsoft User32 library.
% \footnote{\small\url{https://msdn.microsoft.com/en-us/library/windows/desktop/ms648394(v=vs.85).aspx}\normalsize}
    \item \emph{Knowledge about the intended target location},
    which can be challenging in real use.
    % Kinematic models of pointing motions such as Plamondon \etal{}'s~\cite{plamondon1997kinematic} could be used to infer the nature and characteristics (distance, width) of a pointing task using trajectories and speed profiles, although this can be computationally intensive and the accuracy ``in the wild'' of such a method remains unknown.
    Accessibility APIs can detect simple actions like button presses and menu selections, as well as locations of the associated widget~\cite{evans12,skillo,fittswild}, although on a limited subset of widgets.
    The useful heuristic that we propose is to regard the position where the click occurred as the position of the target.
    This does not cause a large error in \methodname's gain update when the size of the target is relatively smaller than the size of the screen (i.e., the distance from the target center point to other points within the target is sufficiently shorter than the distance that the cursor moved) and the user's pointing error rate is low as in general office work.
    % However, if the target is small enough and the user's pointing error rate is low, the location where the click occurred can be approximated as the location of the target.
    % In fact, it is known that the user's pointing error rate is kept low (about 4\%) if there is no serious time limit.
    
    \item \emph{Determining starting point of reaching movement}, which poses a challenge.
    The design of \methodname~has thus far assumed that pointing is a controlled task with a known starting point.
    % In a real systems with uncontrolled pointing tasks, that this assumption is violated.
    However, in an uncontrolled pointing task, it is often difficult to determine when a reaching movement toward a particular target has begun.
    The most widely used heuristic is to consider the beginning of the aimed movement from the submovement containing the highest peak of speed before the click \cite{evans2012taming}.
    This is based on the fact that the first submovement of a general aimed movement has the highest speed peak.
    % The method can be applied in natural (uncontrolled) pointing, if we assume that the last two or three submovements toward a target contribute to the selection, 
% and that they can be retrospectively extracted from logs following a selection.
% This assumption based on the finding that pointing movements are generally composed of a small number of submovements \cite{meyer1988optimality}.
    % However, several possibilities exist that can be explored in future work.
%     Some approaches suggested in previous work, like crowdsourcing \cite{evans12}, are unsuitable for real-time optimization.
% 	Crowdsourcing has been proposed, but this is unsuitable for real-time performance \cite{evans12}.
%     Kinematic models of pointing motions such as Plamondon \etal{}'s~\cite{plamondon1997kinematic} could be used to infer the nature and characteristics (distance, width) of a pointing task using trajectories and speed profiles, although 
%     % this can be computationally intensive and 
%     the accuracy ``in the wild'' of such a method remains unknown.
%     Alternatively, accessibility APIs can detect simple actions like button presses and menu selections, as well as characteristics of the associated widget~\cite{evans12,skillo,fittswild}, although on a limited subset of widgets.
	% If combined with Evans \etal{}'s method, we could obtain both the distance and width components of detected pointing tasks.
% 	% This is presently the most realistic option.
%     This would cause less frequent but more trustworthy gain updates.
    % Even though it does not detect all interface operations, it does so with high accuracy.The consequence of limited scope would be slower convergence. 
    % 
%     % enabled for example by \texttt{libpointing}~\cite{casiez2011no}.
%     This is so far the main obstacle to applying \methodname\ at system level.
%     Most accessibility APIs can only alter the settings already available to the user.
%     Libraries like \texttt{libpointing}~\cite{casiez2011no} are not yet able to alter the gain function of an entire operating system \emph{as is}, but
% 	% describe existing acceleration functions and 
% 	greatly facilitate gain function calculations from input to output.
%     This could be combined with low-level cursor control such as \texttt{Java Robot}s\footnote{\url{https://docs.oracle.com/javase/8/docs/api/java/awt/Robot.html}}, 
% %     but this method remains to be tested.
% 	a successful approach in our current tests.
\end{itemize}

==> new_overview.tex <==
% -------------------------------------------------------------
\section{Overview of Technique}
% -------------------------------------------------------------

\methodname~is based on the three principles of the latest model of human motor planning and motor execution.
First, the most up-to-date models \cite{neilson2005overview, bye2008bump,bye2010bump} describe humans as an intermittent controller \textbf{(principle of intermittent control)}.
This means that the preceding motor plan is updated intermittently as a new motor plan in the course of its execution.
As a result of this intermittent control, submovements are observed in the human motion trajectory during the aimed movement process.

Secondly, it is known that human motion is planned with optimal trajectory \textbf{(principle of optimal control)}.
Assuming optimal control of minimum jerk or acceleration, actual human motion data is well explained.

Third, the execution of human motion is under the influence of signal dependent noise \textbf{(principle of signal dependent noise)}.
The human motor plan outputs the motor command to the muscles and the muscles generate the force, so we can generally assume Gaussian noise with a standard deviation proportional to the magnitude of the acceleration.
This noise is added to the acceleration signal and causes it to be distorted.

% \methodname~is built on the most up-to-date models of human motor planning and motor execution \cite{neilson2005overview, bye2008bump,bye2010bump}.



% \methodname\ is built under the core assumption that \emph{the aiming error of individual pointing submovements is an indication of the inadequacy of the gain function}:
% if a submovement ends before its intended aim point (undershoot), then the gain function was too low and should be increased; 
% if it ends further than its intended aim point (overshoot), then the gain function was too high and should be decreased.
% In both cases, the gain change should be proportional to the amount of aiming error.
% % 
% \methodname\ applies this principle in a speed-dependent manner:
% it treats gain functions as series of gains associated to discrete intervals of input speeds, and only alters a gain when the corresponding ``speed bin'' was used in a pointing task.
% % 
% This principle is summarized in Figure~\ref{fig:principle}.
\begin{figure}[h]
  \centering
  \includegraphics[width=0.95\columnwidth]{figs/principle}
  \caption{\methodname\ improves a discrete gain function by updating gains locally per speed range.
  It segments a movement into submovements to update a profile of aiming errors, which it tries to reduce by adapting the gain response. 
  Here, it is shown how \methodname\ fixes too-low gains at high input speeds, and too-high gains at low input speeds. 
  }
\label{fig:principle}
\end{figure}

% \methodname\ subscribes to a local optimization scheme that assumes that there exists a case-specific optimum gain function (or several optimal gain functions on a Pareto front) for a user performing pointing tasks of certain difficulty and scale ranges, with a given pointing device.
% %
% It also assumes that this function is reachable from an initial constant gain function, by means of a sequence of local updates to the function.
% % 
% Moreover, when updates are based on repeated observations of the user, a reasonable estimate of the optimum function can be obtained despite several sources of variability in the human motor system.

% To estimate the optimum, \methodname\ builds on four assumptions in earlier theories of human motor control:
\begin{figure}[b]
\centering
\includegraphics[width=1.0\columnwidth]{figs/geometry}
\caption{\methodname~assumes that each submovement has an implicit aim point ($D_{aim}$) located at a fraction ($p$) to the remaining target distance ($D_{target}$). In this figure, a submovement is undershooting, which is marked with a positive aiming error $R=(D_{aim}-D_{c})$.}
\label{fig:geometry}
\end{figure}
% 
% % 
% \begin{itemize}
%   % 
%   \item \textbf{Submovement decomposition}: An aimed movement can be divided into one or more submovements \cite{wisleder2007role, crossman1983feedback, meyer1988optimality} using local accelerations and decelerations in the speed profile.

%   \item \textbf{Implicit aim point}: A submovement $i$ has an implicit aim point 
% 	% ($D_{aim}$) <<< that's a distance, not a point 
% 	located at a fraction ($p_i$) of the remaining distance to the target ($D_{target,i}$) at its beginning 
% 	\cite{crossman1983feedback}:
%     %
%   \begin{equation}
%   D_{aim,i}=p_i\cdot D_{target,i}
%   \label{eq:p}
%   \end{equation}
%   %
%   With respect to the aim point, the aiming error $R_i$ of a submovement $i$ is defined as: 
%   %
%   \begin{equation}
%   R_i=(D_{aim,i}-D_{c,i})
%   \label{eq:r}
%   \end{equation}
%   %
%   With $D_{c,i}$ the distance moved during the submovement $i$ (projected, see Figure~\ref{fig:geometry}). 
%   Negative errors indicate overshooting, positive errors indicate undershooting.
%   % 
%   \item \textbf{Stochastic noise}: Due to stochastic noise in the motor system, submovement endpoints are distributed around the center of the aim point \cite{meyer1988optimality}.
%   % 
%   \item \textbf{Intermittent control}: The next submovement starts from where the previous was left \cite{crossman1983feedback, meyer1988optimality}. 
% \end{itemize}


% These assumptions extends tenets of two well-known models of aimed movements.
% % 
% In Crossman and Goodeve's \emph{deterministic iterative corrections model} \cite{crossman1983feedback},
% aimed movements are modeled as series of ballistic, open-loop submovements aimed at a constant fraction ($p$) of the remaining distance to the target.
% However, because empirical data showed large variations in the duration and aim point of these submovements, an extension of the idea was proposed.
% % 
% Meyer's \emph{stochastic optimized submovement model} \cite{meyer1988optimality} assumes that neuromotor noise causes the primary submovement to either undershoot or overshoot the target, which requires a corrective submovement to finally reach the target center.
% It assumes intermittent feedback control, where each submovement is based on the error at the end of the previous one.



% \methodname's objective function is to minimize aiming errors.
% To this end, it applies an iterative search method similar to a gradient descent local optimization scheme. 
% It changes (decrease/increase) the gain function proportionally to the amplitude of aiming error (overshooting/undershooting), and only for the specific speeds actually used in the submovement.

==> study2.tex <==
\section{Study 2: Gain Function for An Emerging Device}

Besides optimizing regularly used input devices,
CD gain adaptation could facilitate the development of novel input devices, such as for VR/AR. 
The objective of Study 2 was to assess \methodname's ability to produce usable gain functions on input devices 
% for which there are no reference function yet --- in this case, a computer vision sensor. 
that were not already hand-tuned for cursor control---in this case, a Leap Motion controller.
% 
This experiment design is similar to Study 1, with only the \golfpart\ condition (no \refpart). 
% 
The cursor was controlled using mid-air hand movements tracked by a Leap Motion controller, (software version 2.3.1+31549).
% 
% In this study we do not have a baseline design, 
We are mainly interested to see if \methodname\ stabilizes to a gain function 
% that improves users performance. <<< for sure, starting from 1
with satisfying performance and user feedback.

\subsection{Participants}
Six paid participants (4 females) were recruited, aged 22 to 30 years old ($\mu$ 25.5 years, $\sigma$ 2.9).
One participant was left-handed.
One participant had 1 year of experience in mid-air pointing, mostly from gaming experience at home with another Leap Motion device.
%AO: what? somebody actually games with these lousy sensors?

\subsection{Design}
% 
The experiment followed a within-subject design with one \emph{gain condition}: \golfpart, which is similar than in the previous study.
The initial gain was set as a flat function with one-to-one mapping ($G[v]=1~\frac{m.s^{-1}}{m.s^{-1}}$) between the speed of index finger and the cursor.
% 
Each participants was to perform 800 trials, which we blocked into 10 \emph{block}s of 80 trials.

\begin{figure}[!t]
\centering
\includegraphics[width=1.0\columnwidth]{figs/timeleap}
\caption{Apparatus and trial completion times in Study 2.}
\label{fig:timeleap}
\end{figure}


\subsection{Task and procedure}
% 
The task (on screen) was the same as in Study 1.
% 
Participants used their dominant hand over a Leap Motion tracker to move the cursor, and their non-dominant hand over the built-in keyboard to click and clutch.
% 
Clicking was performed by pressing the space bar.
% 
The cursor only moved when the C key was held pressed, following the movements of the dominant index finger; clutching was performed by releasing that key, relocating the finger, and resuming pointing by pressing C again.
% 
The finger movements were interpreted as parallel to the display, i.e. on a vertical plane.
This ensured forward/up visual compatibility \cite{phillips2005forward} between hand and cursor movements. 

For each participant, we first calibrated the Leap Motion tracker using its inbuilt calibration software before starting the experiment.
A research assistant then briefly demonstrated the pointing mechanism.
% how the cursor is moved by the tracker according to his finger movement.
%  
Participants sat on a regular office chair that they could adjust, and used a laptop placed on a desk. 
They first filled a preliminary questionnaire asking about their previous experience with mid-air pointing.

During the tasks, participants rested their dominant elbow on a stand aside the desk (at desk height), with the Leap Motion device facing up below their hand and 30 cm below desk height (see Figure~\ref{fig:timeleap}-left).
In effect, their dominant hand rested 30 cm above the Leap Motion tracker, and their elbow was supported to reduce fatigue.
% The Leap Motion tracker was placed 30 cm below the participant's dominant hand and the elbow of participant was supported by a surface to reduce fatigue. 

Participants were instructed to take 10 minutes of practice session with an initial constant gain of 1 before the main part of the experiment started. 
The gain function was not updated during the practice.
% 
During the main session, participants were invited to take breaks every 80 selection tasks.
The experiment lasted about one hour per participant.
% Finally, we recorded all optimization steps of the gain function for analysis.

\subsection{Apparatus}
% 
The experiment was coded in C++ and run on the same computer as in Study 1.
% 
% As the raw output from Leap Motion was already provided in millimeters, the initial flat gain was implemented by considering the resolution of output display with \texttt{libpointing}.
% The initial flat gain was updated after each trial using the \methodname~method.
% 
% , this time using a Leap Motion tracker for input.
% The experiment was coded in C++.
We used the Leap Motion in ``Robust tracking mode'' and smoothened its raw input using the \texttt{1~\euro~filter} \cite{casiez20121}.
Following Casiez \etal{}'s tuning guidelines, we used $10^{-5}$ for minimum cutoff frequency and 0.05 for beta parameter.

The change rate parameter $C$ was set to 3.6$\times10^{-5}$~mm$^{-1}$ after pilot tests; 
this is lower than Study 1 to account for the possible harder learning of the input method, compared to traditional trackpad input.
% in order to prevent unstable fluctuation of the system from its harder learning on mid-air pointing.
We again set the processing noise parameter of the Kalman filter at 0.2, and the sensor noise parameter as 40.0.
The refresh rate of the display was 60 fps.

For dynamic tracking of moving hands, the spatial resolution of Leap Motion controller was reported at around 0.7 mm \cite{weichert2013analysis}.
Therefore, to avoid being sensitive to noise, we discretized the range of input speeds into bins of 1 mm/count (0.06 m/s considering Leap Motion's 60Hz frequency).

\begin{figure}
\centering
\includegraphics[width=1.0\columnwidth]{figs/leapgainfunctions}
\caption{Study 2: \methodname~obtained gain functions with slightly different shapes for different participants.}
\label{fig:gainleap}
\end{figure}
% --------------------------
\subsection{Results}
% 
\subsubsection{Dataset}
% 
In total, 19,271 submovements (4.01 per trial on average) were observed, with 2,219 \emph{interrupted} submovements (11.51\% of all submovements, 0.46 times per trial on average), 7,832 \emph{unaimed} submovements (40.64\% of all submovements, 1.63 times per trial on average), and \emph{non-ballistic} 9,142 submovements (47.44\% of all submovements, 1.9 times per trial on average) according to our criteria.
Note that we detected interrupted submovements in the same way as trackpad study.
The overall average of aim point ($p$) estimated from Kalman filter was 0.94 ($\sigma$ 0.038).

\subsubsection{Trial Completion Time and Error Rates}
% 
Trial completion time was 1.67 second on average ($\sigma$ 0.29).
Completion time varied from 1.94 second ($\sigma$ 0.42) in \block~1 to 1.57 second ($\sigma$ 0.25) in \block~10, for an improvement of 19.1\%.
The effect of \block~on trial completion time was significant (F(9,45)=4.383, p$<$0.001).
Helmert contrast revealed that the improvement in trial completion time was close to being statistically significant for \block~1 (p=0.057) and \block~2 (p=0.052).
Also for \block~7, the improvement showed a weak trend toward significance (p=0.1).
The effect of \block~on error rate was not significant (F(9,45)=0.997, p=0.456).
% The average time of initial \block~was 1.94 second (SD=0.42) and \methodname~showed 22.6\% of improvement in 
% \block~9 (M=1.5 second, SD=0.20), which was the fastest \block.

The mean error rate was 11.3\% ($\sigma$ 7.2). 
Error rates varied from 11.7\% ($\sigma$ 8.8) in \block~1 to 11.0\% ($\sigma$ 9.0) in \block~10.
These high error rates are attributable to a large proportion of relatively small targets in the study, that are at the limit of tracking accuracy which was not fully resolved by filtering.
The larger number of \emph{unaimed} movements in this study (40.64\%) also supports this explanation.
% \mn{Underlined: that explanation is not enough. The point of gain in general, and gain functions in particular, is to link the input range and accuracy to the task characteritics. If the targets are small compared to the input capabilities, then the gain should end up lower.}


% \todo{Good point 2: could we show/discuss the difference between the resulting curves in Study 1 as well? Even saying that they look alike is an interesting result.}

\subsection{Discussion}

% When compared to top performance during 10 minutes of practice with a flat gain function, \methodname~ improved users' performance up to 24\%.
% This benefit is similar to one reported between flat gain and a commercial gain function (up to 24\%) \cite{casiez2011no}.

As in the first study, the gain functions produced by \methodname\ displayed significant performance improvement form the initial condition (here up to 24\%), and reasonable completion times (here around 1.5 second).
% 
Figure \ref{fig:gainleap} shows the evolution of the gain functions that it produced for each participant after each block.
% 
Each function converges. 
The particular shape of a function might reflect the movement specificities and pointing strategy of the participant.

Finally we looked at Fitts' law regression with the data from \block~10.
By averaging over 10-quantiles, we obtained following equation:
% with reasonable throughput of 4.74 bits/s: 
$MT=0.773+0.211\cdot I\!D$, R$^{2}=0.824$.
% 
A previous Fitts' study of mid-air pointing using a Leap Motion device and a hand-tuned acceleration function \cite{liu15} reported similar error rates (10.9\% in average) and a Fitts' law regression of $MT=0.497+0.483\cdot I\!D$ (R$^{2}=0.94$) in a similar range of IDs (1.7 to 5.2 bits).
% Their system was working on a sigmoid CD gain\cite{nancel15} with computer-vision-based click while users were standing, arms-down, and with a large display. 
% They reported a throughput of 2.07 bits/s with similar error rate (10.9\%) than our study: $MT=0.497+0.483\cdot ID, R^{2}=0.94$.
% 
There are a number of differences between the procedures of the two studies: 
in \cite{liu15} participants were standing, the task was performed on a large display, participants had less training (36 trials), clicking and clutching were triggered by hand gestures with inconsistent recognition accuracy, etc.
% 
While these differences prevent formal performance comparison, we obtained overall shorter acquisition times and similar accuracy in the same range of difficulty.
The fact that \methodname\ could produce such a usable gain function in less than 30 minutes of use and with minimal human initialization 
% While we cannot attribute this 129\% improvement exclusively to \methodname, an advantage this large 
warrants further research on automatic gain updating techniques.


